Empowering Sign Language Communication: Integrating Sentiment and Semantics for Facial Expression Synthesis

Translating written sentences from oral languages to a sequence of manual and non-manual gestures plays a crucial role in building a more inclusive society for deaf and hard-of-hearing people. Facial expressions (non-manual), in particular, are responsible for encoding the grammar of the sentence to be spoken, applying punctuation, pronouns, or emphasizing signs. These non-manual gestures are closely related to the semantics of the sentence being spoken and also to the utterance of the speaker's emotions. However, most Sign Language Production (SLP) approaches are centered on synthesizing manual gestures and do not focus on modeling the speakers expression. This paper introduces a new method focused in synthesizing facial expressions for sign language. Our goal is to improve sign language production by integrating sentiment information in facial expression generation. The approach leverages a sentence sentiment and semantic features to sample from a meaningful representation space, integrating the bias of the non-manual components into the sign language production process. To evaluate our method, we extend the Frechet Gesture Distance (FGD) and propose a new metric called Frechet Expression Distance (FED) and apply an extensive set of metrics to assess the quality of specific regions of the face. The experimental results showed that our method achieved state of the art, being superior to the competitors on How2Sign and PHOENIX14T datasets. Moreover, our architecture is based on a carefully designed graph pyramid that makes it simpler, easier to train, and capable of leveraging emotions to produce facial expressions.

==> experiments-and-results.tex <==
\section{Experiments and Results}

To assess our method, we conduct several experiments evaluating different aspects of motion synthesis from audio information. We also compared our method to the state-of-the-art technique proposed by Lee~\etal~\cite{lee2019dancing2music}, hereinafter referred to as D2M. We choose to compare our method to D2M since other methods have major drawbacks that make a comparison with our method unsuitable, such as different skeleton structures in~\cite{ginosar2019gestures}.
%Their method is the closest to ours which we can use without the need of ``greater" modifications. 
Unfortunately, due to the lack of some components in the publicly available implementation of D2M, few adjustments were required in their audio preprocessing step. We standardized the input audio data by selecting the maximum length of the audio divisible by 28, defined as $L$, and reshaping it to a tensor of dimensions $\left(\frac{L}{28}, 28\right)$ to match the input dimensions of their architecture.
%Because their missing audio ``preprocessing'' component  is used to transform the input music into a vector whose shape is a multiple of $28$, explicitly the number of $2D$ coordinates that express the $14$ joints of their adopted skeleton model, we change the music input shape to match the largest multiple of $28$ smaller than the original size of the song. 

The experiments are as follows: \textit{i)} We performed a perceptual user study using a blind evaluation with users trying to identify the dance style of the dance moves. For a generated dance video, we ask the user to choose what style (Ballet, Michael Jackson (MJ), or Salsa) the avatar on the video is dancing; \textit{ii)} Aside from the user study, we also evaluated our approach on commonly adopted quantitative metrics in the evaluation of generative models, such as Fréchet Inception Distance (FID), GAN-train, and GAN-test~\cite{Shmelkov18}. 
%The adaptations were made in both methods. These adjusts will be detailed for each evaluation protocol.sim
%We aim to stress our approach to evaluate how it compares to the \textit{Dancing2Music} framework~\cite{lee2019dancing2music}, state-of-the-art method in motion generation conditioned on music. 

%It is necessary to emphasize that the work of~\cite{lee2019dancing2music} is the one who seeks to solve the closest, to not say the same, problem as ours which we can use without the need of ``greater" modifications. However, due to some missing components in their publicly available implementation of the method, some adjusts to their audio processing step were made in order to use their code to generate results. Because the missing component 'preprocess' is used to transform the input music into a vector whose shape is a multiple of $28$, explicitly the number of $2D$ coordinates that express the $14$ joints of their adopted skeleton model, we change the music input shape to match the largest multiple of $28$ smaller than the original size of the song.

\subsection{Implementation and Training Details}

\paragraph{\textbf{Audio and Poses Preprocessing}}

Our one-dimensional audio CNN was trained for $500$ epochs, with batch size equal to $8$, Adam optimizer with $\beta_1=0.5$ and $\beta_2=0.999$, and learning rate of $0.01$.
%Our set of hyperparameters for the evaluation was for learning rate: $\{0.01, 0.005\}$; for epochs: $\{20, 50, 100, 500\}$, batch size: $\{8, 16,32\}$
Similar to \cite{oord2016wavenet}, we preprocessed the input music audio using a $\mu-law$ non-linear transformation to reduce noise from audio inputs not appropriately recorded. We performed $10$-fold cross-validation to choose the best hyperparameters. %, in these experiments we also evaluate three sound processing models. 

%Them the audio pass through the $1D$ CNN to extract feautures, finally we use a classifier and have the most likely class to the input audio.

In order to handle different shapes of the actors and to reduce the effect of translations in the 2D poses of the joints, we normalized the motion data used during the adversarial GCN training. We managed changes beyond body shape and translations, such as the situations of actors lying on the floor or bending forward, by selecting the diagonal distance of the bounding box encapsulating all 2D body joints $\mbf P_t$ of the frame as scaling factor. The normalized poses are given by: 
\begin{equation}
    \bar{\mbf J_i} = \frac{1}{\delta}\left(\mbf J_i - \left(\frac{\Delta u}{2}, \frac{\Delta v}{2}\right) \right) + 0.5,
    %\bar{\mbf J_i} = \left(\mbf J_i - \left(\frac{\Delta u}{2}, \frac{\Delta v}{2}\right) \right)\frac{2}{\delta} + 0.5,
    %\frac{x-(\frac{x_{max} - x_{min}}{2})}{\epsilon} + 0.5, y_{normalized} = \frac{y- (\frac{y_{max}-y_{min}}{2})}{\epsilon} + 0.5,
    \label{eq:norm}
\end{equation} 
\noindent where $\delta = \sqrt{(\Delta u)^2 + (\Delta v)^2}$, and $(\Delta u, \Delta v)$ are the differences between right-top position and left-bottom position of the bounding box of the skeleton in the image coordinates $(u,v)$. 
%This normalization removes problems of skeleton scale and translation in the image and puts the range of the joint poses for training $\bar{\mbf J}_i \in [0,1]$, {\color{red}without necessarily having at least one joint $\mbf{J}$ in the interval limits.}\RM{This sentence is not clear to me.}\\

\paragraph{\textbf{Training}}

We trained our GCN adversarial model for $500$ epochs. We observed that additional epochs only produced slight improvements in the resulting motions. 
%however the trade-off between gain and cost become less attractive. 
In our experiments, we select $N=64$ frames, roughly corresponding to motions of three seconds at $24$ FPS. We select $64$ frames as the size of our samples to follow a similar setup presented in~\cite{ginosar2019gestures}. Moreover, the motion sample size in~\cite{lee2019dancing2music} also adopted motion samples of $32$ frames. In general, the motion sample size is a power of $2$, because of the nature of the conventional convolutional layers adopted in both~\cite{ginosar2019gestures,lee2019dancing2music}. %, which we use as our temporal upsampling and downsampling layers.
However, it is worth noting that our method can synthesize long motion sequences. We use a batch size of $8$ motion sets of $N$ frames each. 
%Greater batch sizes degraded the model training performance, one of possibilities to this effect was the size of our dataset. 
We optimized the cGAN with Adam optimizer for the generator with $\beta_1=0.5$ and $\beta_2=0.999$ with learning rate of $0.002$. The discriminator was optimized with Stochastic Gradient Descent (SGD) with a learning rate of $2\times10^{-4}$. We used $\lambda = 100$ in Equation~\ref{eq:loss}. Dropout layers were used on both generator and discriminator to prevent overfitting.

\paragraph{\textbf{Avatar Animations}}

As an application of our formulation, we animate three virtual avatars using the generated motions to different music styles. The image-to-image translation technique vid2vid~\cite{wang2018vid2vid} was selected to synthesize videos. We trained vid2vid to generate new images for these avatars, following the multi-resolution protocol described in~\cite{wang2018vid2vid}. %, where the actors  person, that not necessarily know how to dance, is dancing. 
For inference, we feed vid2vid with the output of our GCN. We highlight that any motion style transfer method can be used with few adaptations, as for instance, the works of~\cite{chan2019dance,Gomes_2020_WACV}. 
%\textcolor{purple}{We also train the vid2vid method, without the data of~\cite{guler2018densepose}, because we cannot generate this data using our method.}

%\todo[inline]{Add explanation of the dance styles of the baseline and ours}

%\subsection{Evaluation Setup}

%\todo[inline]{Improve this section - provide a better explanation for stride?}
%\todo[inline]{add something on `However, we manually collect data in a way the styles used by the baseline in their training will be closer than usual'}
%\textcolor{purple}{In order to evaluate our method and a state-of-the-art baseline, we create a second dataset following the same methodology described over this section. This dataset shares the same dance styles of the dataset used to train our method. However, we manually collect data in a way the styles used by the baseline in their training will be closer than usual. The only part of the process of the dataset creation we explained that wasn't applied on the evaluation dataset was the data augmentation using the temporal coherent noise. However we compensate it with a smaller ``stride".}

\subsection{User Study}

%\todo[inline]{explicar a transformação feita nos dados reais para o teste de usuario.}
%\todo[inline]{RAFAEL - explicar como foram calculadas as métricas}



\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{user-study-and-profile.pdf}
    \caption{The plots a), b), c) and d) show the profile distribution of the participants of our user study; The plots e), f), g) and h) show the results of the study. In the plots of semi-circles are shown the results of the user evaluation; each stacked bar represents one user evaluation and the colors of each stacked bar indicates the dance styles (Ballet $=$ yellow, Michael Jackson (MJ) $=$ blue, and Salsa $=$ purple). \textbf{e)} We show the results for all $\mathbf{60}$ users that fully answered our study; \textbf{f)} Results for the users which achieved top $\mathbf{27\%}$ scores and the $\mathbf{27\%}$ which achieved the bottom scores; \textbf{g)} Results for the $\mathbf{27\%}$ user which achieved top scores; \textbf{h)} Results for the $\mathbf{27\%}$ users which achieved worst scores. %Following clockwise order in all plots, the methods are: Ours, Real motion data, and D2M. 
    %\todo[inline]{rework figure left margin to strong}
    }
    \label{fig:user-study-profile}
\end{figure*}

We conducted a perceptual study with $60$ users and collected the age, gender, Computer Vision/Machine Learning experience, and familiarity with different dance styles for each user. Figure~\ref{fig:user-study-profile} shows the profiles of the participants.

The perceptual study was composed of $45$ randomly sorted tests. For each test, the user watches a video (with no sound) synthesized by vid2vid using a generated set of poses. Then we asked them to associate the motion performed on the synthesized video as belonging to one of the audio classes: Ballet, Michael Jackson, or Salsa. In each question, the users were supposed to listen to one audio of each class to help them to classify the video. 
%Because the users were allowed to finish the test at any time, we have $103$ users participating in our study, with $60$ that answered to all questions. %During our study, we ask some informations about the user (\textit{e.g.} Age, Genre, Computer Vision/Machine Learning Experience, Familiarity with different dance styles), these information are shown in Figure~\ref{fig:user-study-profile}. 
The set of questions was composed of $15$ videos of movements generated by our approach, $15$ videos generated by D2M~\cite{lee2019dancing2music}, and $15$ videos of real movements extracted from our training dataset. We applied the same transformations to all data and every video had an avatar performing the motion with a skeleton with approximately the same dimensions. We split equally the $15$ videos shown between the three dance styles.

From Table~\ref{table:results_perceptual} and Figure~\ref{fig:user-study-profile}, we draw the following observations: first, our method achieved similar motion perceptual performance to the one obtained from real data. Second, our method outperformed the D2M method with a large margin. Thus, we argue that our method was capable of generating realistic samples of movement taking into account two of the following aspects: \textit{i)} Our performance is similar to the results from real motion data in a blind study; \textit{ii)} Users show higher accuracy in categorizing our generated motion. Furthermore, as far as the quality of a movement being individual is concerned, Figures~\ref{fig:ours-vs-d2m} and~\ref{fig:ours-results} show that our method was also able to generate samples with motion variability among samples.

We ran two statistical tests,  \textit{Difficulty Index} and \textit{Item Discrimination Index}, to test the validity of the questions in our study. The Difficulty Index measures how easy to answer an item is by determining the proportion of users who answered the question correctly, \ie, the accuracy. On the other hand, the Item Discrimination Index measures how a given test question can differentiate between users that mastered the motion style classification from those who have not. Our methodology analysis was based on the guidelines described by Luger and Bowles~\cite{LugerB16}. Table~\ref{table:results_perceptual} shows the average values of the indexes for all questions in the study. One can clearly observe that our method's questions had a higher difficulty index value, which means it was easier for the participants to answer them correctly and, in some cases, even easier than the real motion data. Regarding the discrimination index, we point out that the questions cannot be considered good enough to separate the ability level of those who took the test, since items with discrimination indexes values between $0$ and $0.29$ are not considered good selectors~\cite{ebel1991essentials}. These results suggest that our method and the videos obtained from real sequences look natural for most users, while the videos generated by \cite{lee2019dancing2music} were confusing.

% \textcolor{purple}{We evaluate our method with a percpetual user study conduced with $XXX$ users. The results of our approach in comparison with our baseline can be seen in Figure ~\ref{fig:ours-vs-d2m} as shown inf Figures~\ref{fig:ours-results},~\ref{fig:ours-ballet},~\ref{fig:ours-salsa} and ~\ref{fig:ours-michael} our approach is capable of produce realistic motion for a human only with an audio as input and the data needed to train an image-to-image translation techinque.}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.9\linewidth]{img/user-study.pdf}
%     \caption{Results for our perceptual study. The semi-circles are the evaluated methods; each stacked bar is one user evaluation; the colors of each stacked bar are the evaluated dance styles (\textit{e.g.} ballet, michael and salsa). \textbf{a)} We show for all $\mathbf{60}$ users that fully answered our study; \textbf{b)} Results for the users which achieved top $\mathbf{27\%}$ scores and the $\mathbf{27\%}$ which achieve the bottom scores; \textbf{c)} Results for the $\mathbf{27\%}$ user which achieve top scores; \textbf{d)} Results for the $\mathbf{27\%}$ users which achieve worst scores. Following clockwise order in all plots, the methods are: Ours, Real and Baseline.}
%     \label{fig:user-study}
% \end{figure}


\begin{table}[t!]
	\centering
	\caption{Quantitative metrics from the user perceptual study.}
	\label{table:results_perceptual}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{@{}crrrrrrrrc@{}}
			\toprule %\hline
			 & \multicolumn{3}{c}{Difficulty Index$^1$ } & \phantom{abc} & \multicolumn{3}{c}{Discrimination Index $^2$} \\ 
			 \cmidrule{2-4} \cmidrule{6-8} 
			\multicolumn{1}{r}{\textbf{Dance Style}}                      & D2M       & \multicolumn{1}{r}{Ours}    & \multicolumn{1}{r}{Real}&& D2M    & \multicolumn{1}{r}{Ours}       & \multicolumn{1}{r}{Real}\\ \midrule %\hline
			\multicolumn{1}{l}{Ballet}    & $0.183$       & 0.943    &  \multicolumn{1}{r}{$\mathbf{0.987}$} && \multicolumn{1}{r}{$\mathbf{0.080}$}     & \multicolumn{1}{r}{$\mathbf{0.080}$}     &0.033\\
			\multicolumn{1}{l}{MJ}    & $0.403$       & 0.760    & \multicolumn{1}{r}{$\mathbf{0.843}$} & & $0.140$     & \multicolumn{1}{r}{$\mathbf{0.240}$}     &0.120 \\
			\multicolumn{1}{l}{Salsa}    & $0.286$       & \multicolumn{1}{r}{$\mathbf{0.940}$}    & 0.820 && $0.100$     & \multicolumn{1}{r}{0.030}    &\multicolumn{1}{r}{$\mathbf{0.180}$}  \\
			\multicolumn{1}{l}{\textit{Average}}    & $0.290$       & 0.881    & \multicolumn{1}{r}{$\mathbf{0.883}$} && $0.106$     & \multicolumn{1}{r}{$\mathbf{0.116}$}    &0.111  \\
			\multicolumn{1}{l}{}    & \multicolumn{3}{c}{\scriptsize{$^1$\textit{Better closer to 1.}}} & & \multicolumn{3}{c}{\scriptsize{$^2$\textit{Better closer to 1.}}} \\
			\bottomrule %\hline
		\end{tabular}
	}
\end{table}

% \todo[inline]{We are not going to add also the overall accuracy plots of Joao and Rafael notebook?}

\subsection{Quantitative Evaluation}
\begin{table*}[t]
	\centering
	\caption{Quantitative evaluation according to FID, GAN-Train, and GAN-Test metrics.}
	\label{table:results_quantitative}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{@{}crrrrrrrrrrrrc@{}}
			\toprule %\hline
			& \multicolumn{3}{c}{FID$^1$ } & \phantom{abc} & \multicolumn{3}{c}{GAN-Train $^2$} & \phantom{abc} & \multicolumn{3}{c}{GAN-Test\* $^3$}\\ 
			\cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
			\multicolumn{1}{l}{\textbf{Dance Style}}                      & \multicolumn{1}{c}{D2M}       & \multicolumn{1}{c}{Ours}    & \multicolumn{1}{c}{Real}&& \multicolumn{1}{c}{D2M}    & \multicolumn{1}{c}{Ours}       & \multicolumn{1}{c}{Real}&& \multicolumn{1}{c}{D2M}    & \multicolumn{1}{c}{Ours}       & \multicolumn{1}{c}{Real}\\ \midrule 
			
			%\hline
			\multicolumn{1}{l}{Ballet}    & $20.20\pm4.41$       & \multicolumn{1}{r}{$\mathbf{3.18\pm1.43}$}    &$2.09\pm0.58$&& $0.36\pm0.15$     & \multicolumn{1}{r}{$\mathbf{0.89\pm0.10}$}     &$0.80\pm0.12$ && $0.07\pm0.04$     & \multicolumn{1}{r}{$\mathbf{0.80\pm0.14}$}     &$0.77\pm0.11$\\  
			\multicolumn{1}{l}{MJ}    & $\mathbf{4.38\pm1.94}$       & \multicolumn{1}{r}{$8.03\pm3.55$}    &$5.60\pm1.42$& & $0.34\pm0.15$     & \multicolumn{1}{r}{$\mathbf{0.60\pm0.13}$}     &$0.59\pm0.04$ && $\mathbf{0.70\pm0.14}$     & \multicolumn{1}{r}{$0.46\pm0.18$}     &$0.60\pm0.09$ \\
			\multicolumn{1}{l}{Salsa}    & $12.23\pm3.20$       & \multicolumn{1}{r}{$\mathbf{4.29\pm2.38}$}    & $2.40\pm0.75$ && $\mathbf{0.32\pm0.17}$     & \multicolumn{1}{r}{$0.31\pm0.11$}    &$0.50\pm0.16$   && $0.26\pm0.14$       & \multicolumn{1}{r}{$\mathbf{0.96\pm0.11}$}    & $0.90\pm0.06$   \\
			\multicolumn{1}{l}{\textit{Average}}    & $12.27\pm7.27$       & \multicolumn{1}{r}{$\mathbf{5.17\pm3.33}$}    & $3.36\pm1.86$ && $0.34\pm0.16$     & \multicolumn{1}{r}{$\mathbf{0.60\pm0.26}$}    &$0.63\pm0.17$  && $0.34\pm0.29$       & \multicolumn{1}{r}{$\mathbf{0.74\pm0.25}$}    & $0.76\pm0.15$  \\
			
			
			\multicolumn{1}{l}{}    & \multicolumn{3}{c}{\scriptsize{$^1$\textit{Better closer to 0.}}} & & \multicolumn{3}{c}{\scriptsize{$^2$\textit{Better closer to 1.}}} & & \multicolumn{3}{c}{\scriptsize{$^3$\textit{Better closer to 1.}}}\\
			\bottomrule %\hline
		\end{tabular}
	}
\end{table*}

For a more detailed performance assessment regarding the similarity between the learned distributions and the real ones, we use the commonly used Fr\'echet Inception Distance (FID). We computed the FID values using motion features extracted from the action recognition ST-GCN model presented in~\cite{yan2018spatial}, similar to the metric used in \cite{yan2019convolutional,lee2019dancing2music}.
%adapt the work of \cite{yan2018spatial} to use it as a action recognition method based on graph convolutional neural networks. 
We train the ST-GCN model $50$ times using the same set of hyperparameters. The trained models achieved accuracy scores higher than $90\%$ for almost all $50$ training trials. The data used to train the feature vector extractor was not used to train any of the methods evaluated in this paper. Table~\ref{table:results_quantitative} shows the results for the FID metric.

% Our method leads the performance for all dance styles, and according to the Wilcoxon Signed Rank statistical test, our method presented the same performance of D2M for the Salsa.



% \todo[inline]{COUTINHO - falar sobre o teste estatístico, incluir citação. Melhorar explicação- what values exactly? what distances? specify}
%\todo[inline]{Since the values we obtain in our test present great variance, we perform the Wilcoxon signed-rank test. With that we show that the two distributions of distances collected in our tests are disjoint with $p-value$ of $X$.}

We also computed the GAN-Train and GAN-Test metrics, two well-known GAN evaluation metrics~\cite{Shmelkov18}. To compute the values of the GAN-Train metric, we trained the ST-GCN model in a set composed of dance motion samples generated by our method and another set with generated motions by D2M. Then, we tested the model in the evaluation set (real samples). The GAN-Test values were obtained by training the same classifier in the evaluation set and tested in the sets of generated motions. For each metric, we ran $50$ training rounds and reported the average accuracy with the standard deviation in Table~\ref{table:results_quantitative}. Our method achieved superior performance as compared to D2M. 

We can also note that the generator performs better in some dance styles. Since some motions are more complicated than others, the performance of our generator can be better synthesizing less complicated motions related to a particular audio class related to a dance style. For instance, the Michael Jackson style contains a richer set of motions with the skeleton joints rotating and translating in a variety of configurations. The Ballet style, on the other hand, is composed of fewer poses and consequently, easier to synthesize.


%Finally we highlight in Table~\ref{table:results_quantitative}, the method with best results in average for all metrics.

%Please remark that GAN-Test results reported in Table~\ref{table:results_quantitative} were obtained by training the classifier in the validation dataset, and tested on both training dataset and synthesized ones for both methods (D2M and ours). This modification was required in the metric, since the D2M has never seen the data used for training. Finally we highlight in Table~\ref{table:results_quantitative}, the method with best results in average for all metrics. %, ignoring the standard deviation, 

%\todo[inline]{The GAN-Test and GAN-Train are not very clear to me. This paragraph should be improved.}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{our-vs-baseline.pdf}
    \caption{Results of our approach in comparison to D2M \cite{lee2019dancing2music} for \textit{Ballet}, the dance style shared by both methods.}
    \label{fig:ours-vs-d2m}
\end{figure}

\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.72\linewidth]{ours-results.pdf}
    \caption{Qualitative results using audio sequences with different styles. In each sequence: First row: input audio; Second row: the sequence of skeletons generated with our method; Third row: the animation of an avatar by vid2vid using our skeletons.}
    \label{fig:ours-results}
    \vspace*{\floatsep}
    \centering
    \includegraphics[width=0.73\linewidth]{ours-results_demonstration.pdf}
    \caption{Experiment 1 shows the ability of our method to generate different sequences with smooth transition from one given input audio composed of different music styles. Experiment 2 illustrates that our method can generate different sequences from a given input music.}
    \label{fig:ours-results_2}
\end{figure*}

%\todo[inline]{In table~\ref{table:results_quantitative} perhaps use only 1 or 2 decimal value}


\subsection{Qualitative Evaluation}

Figures~\ref{fig:ours-vs-d2m}, \ref{fig:ours-results}, and \ref{fig:ours-results_2} show some qualitative results. We can notice that the sequences generated by D2M presented some characteristics clearly inherent to the dance style, but they are not present along the whole sequence. For instance, in Figure~\ref{fig:ours-vs-d2m}, one can see that the last generated skeleton/frame looks like a spin, usually seen in ballet performances, but the previous poses do not indicate any correlation to this dance style. Conversely, our method generates poses commonly associated with ballet movements such as rotating the torso with stretched arms. 



Figure~\ref{fig:ours-results} shows that for all three dance styles, the movement signature was preserved. Moreover, the \textit{Experiment 1} in Figure~\ref{fig:ours-results_2} demonstrates that our method is highly responsive to audio style changes since our classifier acts sequentially on subsequent music portions. This enables it to generate videos where the performer executes movements from different styles. Together these results show that our method holds the ability to create highly discriminative and plausible dance movements. Notice that qualitatively we outperformed D2M for all dance styles, including for the Ballet style, which D2M was carefully coined to address. \textit{Experiment 2} in Figure~\ref{fig:ours-results_2} also shows that our method can generate different sequences from a given input music. Since our model is conditioned on the music style from the audio classification pipeline, and not on the music itself, our method exhibits the capacity of generating varied motions while still preserving the learned motion signature of each dance style.  

%\todo[inline]{Need revision figure 7 se vai usar esqueletos ou vid2vid}




%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.9\linewidth]{img/ours-results-ballet.pdf}
%    \caption{Results of our method for \textit{ballet} class.}
%    \label{fig:ours-ballet}
%\end{figure}



%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.9\linewidth]{img/ours-results-salsa.pdf}
%    \caption{Results of our method for \textit{salsa} class.}
%    \label{fig:ours-salsa}
%\end{figure}


%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.9\linewidth]{img/ours-results-michael.pdf}
%    \caption{Results of our method for \textit{michael} class.}
%    \label{fig:ours-michael}
%\end{figure}


% \subsection{Qualitative Results}

% \todo[inline]{Explain adaptations on the baseline, audio preprocess, diffenrt skeleton}
% \todo[inline]{Explain the adaptations on our methdo to make the qunatitative metric more fair, drop joints}
% \todo[inline]{Highligth that our method generate skeletons with more information (more joints), so it is a more complicated task}
% \todo[inline]{explain results of vid2vid bellow the known - because of lack of data}
% \subsection{Training, Baseline and Evaluation Set-up}
% \todo[inline]{Explain the competitor set-up. And then please explain carefully the adopted metrics.}
% \todo[inline]{Add sugestions to see our suplementary video.}


% \todo[inline]{explain FID and our classifier}
% \subsection{Qualitative Results}

% \todo[inline]{explicar como foi feito o estudo com o usuario}
% \todo[inline]{RAFAEL - escrever quants pessoas tinham no dataframe usado para achar as metricas da tabela}
% \todo[inline]{talvez adicionar uma tabela com algumas estatiscas do estudo de usuario - quants pessoas fizeram, quants responderam tudo, quants consideramos, etc}


% \subsubsection{Quantitative Results}





% \todo[inline]{RAFAEL - escrever quants pessoas tinham no dataframe usado para achar as metricas da tabela}

% \todo[inline]{referenciar as figuras do user study}
% \todo[inline]{referenciar as tabelas do user study}
% \todo[inline]{precisa de revisao}



% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{img/boxplot.png}
%     \caption{Boxplot FID analysis.}
%     \label{fig:boxplot-fid}
% \end{figure}









% In this Chapter the preliminary results are shown and detailed, as well the expected results for the project. The preliminary results shown the stage of the project, and according to the work plan presented in the Table \ref{tab:schedule} the development of the project until early June of 2019. Also the expected results of the project will be discuss and the possibilities to the project future. 

% % \todo[inline]{improve preliminary results}
% \section{Preliminary Results}
% As preliminary results a novel dataset composed of 21 YouTube videos that takes about 5365 seconds or 89 minutes approximately of video, with the 2D human poses estimates calculated for every second and the audio with the spectrogram of it. And as the videos are from a YouTube channel famous for doing this kind of video, we can possible grow this dataset as far as it would be needed.

% Another preliminary result is a initial implementation of the model architecture presented in Figure ~\ref{fig:method}, however this initial implementation is much simpler than the one present in previous chapter. In this first implementation we explore the use of just one 2D human pose to each second (batch of the dataset), because the 2D joints of the human pose are in $\mathbb{R}^{3}$. The third and last dimension of the data is its confidence, and so we can extract the most confident pose in the that second (batch), and use that pose as a \textit{``key pose''} for that second (batch). With this \textit{``key pose''} we are trying to feed a model able of minimize the Equation \ref{eq:loss}, where $p'$ is the model predicted 2D human \textit{``key pose''}, and $p$ is the ground truth \textit{``key pose''} for that sound. We iterate over the $25$ joints to minimize the error between the joints predictions.

% e
% After this prediction of the model we will explore the possibility of interpolate these \textit{``key poses''} and create a temporally coherent movement to animate a virtual avatar.

% % \todo[inline]{improve expected results}
% \section{Expected Results}

% The expected results are that from an generic audio file, as example a new trending hit from a famous artist that do not have an unique dance performance designed yet, or even do not have a video clip for the music. Taking the music with the audio, and synthesize a set of human poses that represent that sound. Also is expected that the set of human poses synthesized by the method to be temporally coherent, and also to be possible to get that set and make a virtual avatar replicate the motion.

% In the end two points must be highlighted in the expected results of the project. \textit{\textbf{i))}} The results of the method should be temporally coherent, even when the input is an audio file with more then 1-second of duration. And \textit{\textbf{ii)}} The method should be able of from an audio that anyone ever has listen to, create a reasonable (qualitatively speaking) set of human poses to represent the motion with that audio.

% In the end two points must be highlighted in the expected results of the project. \textit{\textbf{i))}} The results of the method should be temporally coherent, even when the input is an audio file with more then 1-second of duration. And \textit{\textbf{ii)}} The method should be able of from an audio that anyone ever has listen to, create a reasonable (qualitatively speaking) set of human poses to represent the motion with that audio.
